Network extraction by routing optimization

Routing optimization is a relevant problem in many contexts. Solving directly this type of optimization problem is often computationally unfeasible. Recent studies suggest that one can instead turn this problem into one of solving a dynamical system of equations, which can instead be solved efficiently using numerical methods. This results in enabling the acquisition of optimal network topologies from a variety of routing problems. However, the actual extraction of the solution in terms of a final network topology relies on numerical details which can prevent an accurate investigation of their topological properties. In this context, theoretical results are fully accessible only to an expert audience and ready-to-use implementations for non-experts are rarely available or insufficiently documented. In particular, in this framework, final graph acquisition is a challenging problem in-and-of-itself. Here we introduce a method to extract networks topologies from dynamical equations related to routing optimization under various parameters' settings. Our method is made of three steps: first, it extracts an optimal trajectory by solving a dynamical system, then it pre-extracts a network and finally, it filters out potential redundancies. Remarkably, we propose a principled model to address the filtering in the last step, and give a quantitative interpretation in terms of a transport-related cost function. This principled filtering can be applied to more general problems such as network extraction from images, thus going beyond the scenarios envisioned in the first step. Overall, this novel algorithm allows practitioners to easily extract optimal network topologies by combining basic tools from numerical methods, optimization and network theory. Thus, we provide an alternative to manual graph extraction which allows a grounded extraction from a large variety of optimal topologies.

==> sections/Choosing_the_best_representation.tex <==
% !TEX program = pdflatex
% !TEX root = main.tex

\subsection{Choosing the best representation to our problem}

The reason why we decided to use the graph representation defined in Section \ref{theory_for_graph_extraction_implem} instead of the one of the Section \ref{graph2} is justified in terms of the connectivity of the generated graphs. Using the latter we impose that $deg(v)\leq 3,\ \forall v\in G$. This combined with the topology of the grid makes it more likely to generate disconnected graphs, that do not represent properly the connected solutions obtained by the DMK solver. 

On the other hand, the representation defined in Section \ref{graph3} even though experimentally seems to reduce the disconnected graphs, it increases the presence of triangles which in principle get us further of one of our main objectives: removing non-optimal structures. Using an extra simplification step for this graph representation (like the ones described in the following sections) is part of our future plans. 

\subsection{Useful graph concepts}

\subsubsection{Graph connectivity}\label{connectivity}

The standard definition\footnote{\href{http://diestel-graph-theory.com/index.html}{Graph Theory.}} of a \textit{connected graph} is:  A graph $G$ is called \textit{connected} if it is non-empty and any two of its vertices are linked by a path in $G$. Instead of \textit{not connected}, we usually say \textit{disconnected.}

Regarding to our transportation problem, this definition is not appropriated. We are interested in finding graph representations that are connected in some subset of the domain and disconnected in some other. This \textit{partial connectivity} is required to capture the main transportation properties of our solutions. We dedicate the rest of this section to define this property. 

Remember that one of our goals is to find ways of connecting different set of sources and sinks. This means that some \textit{paths} from the support of $f^+$  ($\text{supp}(f^+)$) to the support of $f^-$ ($\text{supp}(f^-)$) must be found. This information is stored in the solutions $(\mu^*, u^*)$ given by the DMK solver. Therefore, we need to be careful when extracting graphs out of them. Figure \ref{extracted_graphs} shows three different graphs extracted from the same pair $(\mu^*, u^*)$ but different values of $\delta.$ 



\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.60\textwidth}
        \includegraphics[width=\textwidth]{figs/uniform_tdens+beta=1p1.png}
        \caption{$\mu^*$ for uniform initial transport density}
        \label{uniform}
    \end{subfigure}
    
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/3Gpc0_graph1.png}
        \caption{$G_1$: $\tau = 0.001$ }
        \label{g1}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/3Gpc1_graph1.png}
        \caption{$G_2$: $\tau = 0.01$}
        \label{g3}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/3Gpc10_graph1.png}
        \caption{$G_3$: $\tau = 0.1$}
        \label{g4}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \caption{Extracted graphs for different values of $\delta$}\label{extracted_graphs}
\end{figure}



As it is clear, values of $\delta$ too close to $\underset{x}{\min} \ \mu^*(x)$ (as in Figure \ref{g1}) will give us graphs $G_\delta$  showing roughly the  same information provided by the solution $\mu^*$. On the other hand, values of $\delta$ too close to $\underset{x}{\max} \ \mu^*(x)$ will lead to very disconnected graphs, and specifically, to broken paths connecting sources and sinks. Thus, having values of $\delta$ far from $\underset{x}{\min} \ \mu^*(x)$ but not too close to $\underset{x}{\max} \ \mu^*(x)$ is necessary to keep these paths unbroken. 

In order to pursuit this trade-off in an easier way, we will state more precisely the framework and the problem under consideration. 

Let $(\mu^*,u^*)$ be the solution of the DMK equations for a set of initial conditions. Denote by $G^*_\delta$ to the graph extracted using the algorithm described in Section \ref{theory_for_graph_extraction_implem}, for $\delta>0.$ Namely, $G^*_\delta$ is equal to $(V,E,w,p)$, where $w$ is an edge-weight function of the optimal transport density and $p$ is a node-weight function related to the location of the nodes in the domain $\Omega$. For a given $\delta>0,$ we define the \textit{exterior of $G^*_\delta$ with respect to $f^+$ and $f^-$}  as a subgraph of $G^*_\delta$  such that $f^+(v)=0$ and $f^-(v)=0$, $ \forall \ v\in V(B).$ We denote it as $O_{f^+,f^-}$ and we rename it as the \textit{exterior}, as long as there is not ambiguity.   We define a \textit{main branch} $B$ of $G^*_\delta$ as a component\footnote{A maximal connected subgraph of $G$ is a \textit{component} of $G$.} of $O_{f^+,f^-}$.  The collection of main branches $B$ is called the \textit{set of branches} of $G^*_\delta$ and it is denoted by  $\mathcal{B}$. 

%For instance, the number of main branches of the graphs $G_1, \ G_2$ and $G_3$ are ?, ? and  ?, resp.,  (see Figure (?)).

Define now the \textit{transport tale w.r.t $f^+$} (or \textit{transport tale w.r.t $f^-$}) of a main branch $B\in \mathcal{B}$ as the set of vertices $\text{tail}^+(B)\subset V(B)$ (or $\text{tail}^-(B))$ such that for every $v\in V(B)$, there exists a $w$ such that $w$ is a neighbour of  $v$ in $G^*_\delta$  and $f^+(u)>0$ (or $f^-(u)>0$). In many cases, we will refer to the transport tale w.r.t $f^+$ ($f^-$) of a main branch $B$ as the positive (negative) tale of $B$.  Note that for a main branch $B$ it is possible to have $\text{tail}^+(B)=\varnothing=\text{tail}^-(B)$ %(see Figure ()). 

\textbf{Conjecture:} If $\mathcal{B}=\{B_1,...,B_n\}$, then

\begin{enumerate}
    \item there exists $I\subset \{1,2,...,n\}$, s.t., $\text{tail}^+(B_i)\neq \varnothing, \ \forall i\in I$ and

$$
\bigcup_{B_i\in \mathcal{B}} \text{tail}^+(B_i)=\bigcup_{i \in I} \text{tail}^+(B_i)
$$
\item there exists $J\subset \{1,2,...,n\}$, s.t., $\text{tail}^-(B_i)\neq \varnothing, \ \forall i\in J$ and

$$
\bigcup_{B_i\in \mathcal{B}} \text{tail}^-(B_i)=\bigcup_{i \in J} \text{tail}^-(B_i)
$$
\item $|I|=|J|\leq |\mathcal{B}|.$
\end{enumerate}
\textit{Proof.} We are working on that. It could be a consequence from the definition of tale and the balance equations. 

The number $|I|$ is called the \textit{branching index} $b(G^*_\delta)$ of $G^*_\delta$.   

Some remarks:

\begin{enumerate}
    \item Note that it seems that for $\delta_1 \leq \delta_2,$ it is true that $|\mathcal{B}_{\delta_1}|\leq |\mathcal{B}_{\delta_2}|,$ leading to $b(G^*_{\delta_1})\leq b(G^*_{\delta_2})$. 
    \item  It is clear that for a given $\delta$, $b(G^*_\delta)\geq 0.$ Figure (?) shows an example of $b(G^*_\delta)=0$. 
\end{enumerate}

With this new notation we are able to state the first draft of the problem in the following way:
$$ 
\text{\textbf{Problem 1:} For a fixed pair $(\mu^*,u^*)$, find $\delta>0,$ s.t. $b(G^*_\delta)=|\mathcal{B}|.$}
$$

In other words, we would like to find $\delta$ such that the number of positive tails (and negative tails) is equal to the number of branches $\mathcal{B}$. If this is true, then we can be sure that the chosen threshold $\delta$ is not breaking the paths between the source and the sink. Intuitively, we want to find $\delta$ such that the graph generated once we connect all the positive tails among themselves and the negatives tails among themselves is \textit{connected} in the standard way. 

It should be clear that the solution of the Problem 1 is not unique. On the other hand, if $\delta^*$ is a solution, it is true that if $ \delta\leq \delta^*,$ then $\delta$ is also a solution (see Remark 1).  \textit{Very small} solutions $\delta$ will lead to more links and therefore, as we mentioned before, to graphs carrying essentially the same information shown by $(\mu^*,u^*)$. This way, it is clear that larger solutions are preferred. This takes us to the second and last draft of the problem related to the connectivity:
$$
\begin{array}{rl}
\text{\textbf{Problem 2:}} & \text{For a fixed pair } (\mu^*,u^*), \text{ define }  \\
&\mathcal{D}=\{\delta>0: \delta \text{ is a solution of Problem 1} \}.\\
&\text{Find $\delta^*$, s.t., $\delta^*=\max \mathcal{D}$.}
\end{array}
$$

Solutions of Problem 2 are unique and are totally dependant on $(\mu^*,u^*)$. Thus, for each solution $(\mu^*,u^*)$ found by the DMK solver, we can define properly the graph $G^*:=G^*_{\delta^*}$ associated to such solution and generated using algorithm in Section \ref{theory_for_graph_extraction_implem}.

It is worth mentioning that all the definitions shown before can be restated for any transport function $\mu$ instead of using the optimal ones. The analysis of the set of main branches $\mathcal{B}_k$ computed for the element of the sequence $\{(\mu_k,u_k)\}_k$ generated by the DMK solver is part of our future plans. 

 
\subsubsection{Betweenness centrality}\label{betweenness_centrality}

Assume that $G$ is a unweighted and connected graph of the form $(V,E)$. For every pair of nodes $(s,t)\in V(G)^2$, a path $P$ connecting $s$ and $t$ is a sequence $(v_1,v_2,...,v_n)\in V(G)^n$ where $v_1=s,$ $v_n=t$ and s.t., the labels are given by order of appearance when moving from $s$ to $t$ on $G$.Depending on the structure of $G$, it is possible to have more than one path $P$ connecting $s$ and $t$.  The set of all the paths from $s$ to $t$  is $P[s,t]$.  We say that $n-1$ is the \textit{length} of $P$ (the number of edges in the path) and in general, we denote it by $l(P)$. The length of path helps us to find \textit{better} ways of connecting two nodes. To get a clearer idea of this notion, consider the following optimization problem: 
$$
\text{\textbf{Problem 3:}}\ \ \text{For } (s,t)\in V(E)^2, \text{ find } P\in P[s,t]  \text{ s.t., }  l(P) \text{ is minimum. }
$$

Solutions of Problem 3 are called \textit{shortest paths} connecting $s$ and $t$. They are useful in many graph problems (ref?). The number of elements in the set
$$
\mathcal{S}_{s,t}:=\{P\in P[s,t]: P \text{ solves Problem 3 }  \}
$$
is denoted by $\sigma[s,t]$. 

We say that a path $P=(s,v_2,...,v_{n-1},t)$ contains $v\in G$ (i.e., $v\in P$) if there is some $j\in \{2,3,..,n-1\}$, s.t., $v_j=v$.  The set of all the paths from $s$ to $t$ going through $v$ is $P_v[s,t]$. The number of elements in the set

$$
\mathcal{S}^v_{s,t}:=\{P\in P[s,t]: P \text{ solves Problem 3 and } v\in P \}
$$

is denoted by $\sigma_v[s,t]$. Paths $P\in \mathcal{S}^v_{s,t}$ are called \textit{shortest paths connecting $s$ and $t$ through $v$}.

We define the \textit{betweenness centrality}\footnote{\href{https://en.wikipedia.org/wiki/Betweenness_centrality}{Betweenness centrality}.} of $v$ as
\[
\text{bc}(v)=\! \! \! \underset{\begin{subarray}{1} (s,t)\in V(G)^2:\\  \ \ s\neq v \neq t\end{subarray}}{\sum} \! \! \! \! \dfrac{\sigma_v[s,t])}{\sigma[s,t]}
\]

Intuitively,  $\text{bc}(v)$ tells how \textit{important} $v$ is in terms of the shortest connections. If $\text{bc}(v)$ is small, then a few connections are taking $v$ into account when linking all pairs $(s,t)$.   Higher values imply a higher dependence on $v$ for the creation of paths in $G$.

Note that if we redefine $G$ as a weighted graph $(V,E,w)$, where $w:E\rightarrow \mathbb{R}^+$ is the function $w(e)=1, \ \forall e\in E, $ then Problem 3 can be restated as
$$
\begin{array}{rc}
\text{\textbf{Problem 4:}}&\ \ \text{For } (s,t)\in V(E)^2, \text{ find } P=(v_1,..,v_n)\in P[s,t]  \text{ s.t., } \\ &\underset{1\leq i\leq n-1}{\sum} \!\!\!\! w(\{v_i,v_{i+1}\})  \text{ is minimum. }
\end{array}
$$

Thus, it is natural to define the optimization problem mentioned before (Problem 3) for more general weighted and connected graphs $G=(V,E,w)$, with arbitrary edge-weight functions, through Problem 4. Solutions of this problem are called \textit{weighted shortest paths connecting $s$ and $t$}.  

Note that the function $\text{bc}:V\rightarrow \mathbb{R}$ allows us to define a new weighted graph $G'$ from another weighted graph $G=(V,E,w)$ as $G'=(V,E,\text{bc})$. This way, we can go from edge-weighted graphs to node-weighted graphs. A useful application of this transformation will be explained in Section \ref{steiner_problems} about Steiner Problems. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> sections/Connecting_two_models.tex <==
% !TEX program = pdflatex
% !TEX root = ../main.tex


\paragraph{On the connections between the two models}

How does the PP dynamical problem connects with DMK? As proposed in \cite{facca2016towards}, 
under certain conditions, the solutions for a mold in the maze are equivalent to an optimal transportation problem. In the following, we summarize such connections.

Considering the dynamics that explain how the plasmodium of Physarum can solve a maze, proposed by Tero et. al. \cite{tero2007mathematical}, we have
\begin{equation}
\begin{split}
Q_{ij} & = D_{ij}\frac{(p_i-p_j)}{L_{ij}},  \\ 
\frac{d}{dt}D_{ij}& = f(|Q_{ij}|) - rD_{ij}, \\
\sum_{i} Q_{ij} &= b_{ij},  \\
Q_{ij}(t = 0)& >0
\label{ppdd}
\end{split}
\end{equation}
as described in previous sections, where $Q_{ij}$ computes the mass flow between nodes $i$
and $j$ through edges with diameter $D_{ij}$, $b_{ij}$ indicates the position of a source/sink node, and $p_i$ ($p_j$) is the hydrostatic pressure in the node $i$ ($j$).
 
On the other hand, the continuous set equations for dynamical Monge-Kantorovich are

\begin{equation}
\begin{split}
	-\nabla \cdot (\mu(t,x)\nabla u(t,x)) &= f(x) \\
\frac{\partial \mu(t,x)}{\partial t} &= \mu(t,x) (|\nabla u(t,x)| - 1) \\
\int_\Omega f(x)dx &= 0 \\
\mu(0,x) &= \mu_0(x) > 0
\label{ddmk}
\end{split}
\end{equation}

Those dynamics are equivalents at the limit for large times ($t\rightarrow \infty$), as conjectured in \cite{facca2016towards}. In this limit, finding a solution for PP is an application to the numerical solutions of an optimal transportation problem. Taking into account a more general setting, we have

\begin{equation}
\frac{\partial \mu(t,x)}{\partial t} = (\mu(t,x)\nabla u(t,x))^{\beta} - \kappa(x)d(t)(\mu(t,x))^\alpha,
\end{equation}
where the transport configuration settings will be different depending on the values of $\beta$. For instance, when $\beta = 1$, the mass will be transported in a straight line (see figure). 



Depending on the different values for $\beta$, we can be in different configurations for a transportation problem. In $(a)$ ($\beta$ < 1), the converged solution is such that the mass avoids congestion, in $(b)$ ($\beta = 1$)is shortest path-like, since the mass goes in a straight line from source to sink, while in $(c)$ and $(d)$, where both $\beta > 1 $ the solution has a setting from a branch transportation problem-like.

Tracing the equivalence relations between eq. \ref{ppdd} and \ref{ddmk}, we get 
 \begin{equation}
 	D_{ij}(t) \longrightarrow \mu(t,x),
 \end{equation}
which implies that on the transition from a discrete to a continuous picture, the edges diameter (we can think that those edges are like small cylindrical channels with a given diameter where the mass is passing trough) are described by an initial distribution $\mu$. Thus, this initial distribution is describing how the edges are changing on time until the solution reaches convergence.

Regarding the mass flow, one can notice that the amount of mass going from node $i$ to node $j$ is stored on the quantity $Q_{ij}$, which in the continuous scenario is given by the product of the density distribution $\mu(t,x)$ with the gradient of the potential $\nabla u(x,t)$, which leads to
\begin{equation}
	 Q_{ij}(t) \longrightarrow \mu(t,x)|\nabla u (t,x)|.
\end{equation}

The third correspondence is given by the positions of sources and sinks on space. The sources or sink nodes ($i$ or $j$), with associated hydrostatic pressure $p_i$, $p_j$, are equivalents to the source and sink functions $f(x)$ (respectively, $f^{+}(x)$ and $f^{-}(x)$), 
\begin{equation}
    b_{ij} \longrightarrow f(x).
\end{equation}

The last correspondence here refers to the boundary conditions of each dynamics. While in the graph, the injection term for initial times must be positive, in the continuous case, the amount of mass that needs to be send from a source to a sink, must be also positive. From a more intuitive perspective, if the initial distributions are equal to zero, means that no mass is being transported. In this case,

\begin{equation}
    Q_{ij}(t=0) \longrightarrow \mu(0,x) = \mu_0(x)>0 .
\end{equation}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> sections/From_a_theoretical_point.tex <==
% !TEX program = pdflatex
% !TEX root = ../main.tex

%\paragraph{Using both side nodes and links as neighbors}
%



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:



==> sections/Nefi.tex <==

%\begin{document}
%\title{Drafts}
%\author{ \textcolor{red}{(We should put an order for the authors here)}}
%\date{October 2019}
%\maketitle
%%\section{Alternative paths for the network extraction}

%\section{NEFI}

NEFi is a platform created in 2015 by M. Dirnberger et.al. \cite{dirnberger2015nefi} that combines elements of computer vision, image processing and graph theory in order to make the process of graph extraction easier. Essentially, the user can give any image as input that the software will give a clean graph as output.

Nefi relies on OpenCV \cite{dirnberger2015nefi}, a well-known library from computer vision. The main steps until the graph extraction includes preprocessing, segmentation, graph detection and graph filtering. The first one prepares the input image to the second one, trough Gaussian and median blurring, denoising and bilateral filter; in the segmentation collection step, the main goal is to separate the image foreground from the remaining image. In the last two steps, the algorithm detects nodes and edges in the image, gives the graph as final output, while make a filtering for remove parts in the graph that are not from interest. This step was designed such that several algorithms can be used interchangeably, like basic tresholding algorithms as well as segmentation routines. It is also mentioned that there is no recipe that will fit best for each image, which gives freedom to the user for choosing whatever is more convenient to the problem.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/Images_Daniela/Initial_image_NEFI.png}
    \caption{Input of a parabolic mass distribution generated on VisIt. Threshold for this image was equal to 0.1.}
    \label{fig:my_label}
\end{figure}
Here we preprocess the images that are solutions from a continuous setting, and we aim to obtain a network as clean as possible. This input image is generated at VisIt, when the solver reaches the convergence.


We used the following configuration for the input images: color table in black and white continuous, triangles in a log scale with a nodal shape. The threshold was often adjusted for each flag differently, where the average value was often around $0.1$. %A second round of tests included different color scales...

\begin{figure}[h!]
  \begin{subfigure}{0.5\textwidth}
    \includegraphics[width=0.9\textwidth]{figs/Images_Daniela/Skel_from_nefi.png}
  \end{subfigure}
  \begin{subfigure}{0.5\textwidth}
    \includegraphics[width=0.9\textwidth]{figs/Images_Daniela/Graph_guo_hall_graph_detection_Parabola_1001.png}
  \end{subfigure}
  \caption{One of the steps before the graph extraction is the skeleton generation (left). The final graph is given by the red line that connects the blue points (right).}
\end{figure}

The graph detection collection takes a segmented image and detect the nodes and edges of the graph. Starting from the thinning, that is  of reducing the segmented foreground such that every line is a single pixel thick and preserving connectivity properties between foreground and background pixels, giving a skeleton as output. They implemented the Guo and Hall schemes. On the skeleton, they detect the position of the nodes, although the maximum number of connectivity for a node is equal to $4$. By performing a variant of breadth they find the edges between the nodes. This has Network as backend.

The last step is the graph filtering. Here, if the network in the input image is large, then the final graph will have a large connected component. The filtering strategy is essentially remove everything that is not in the largest component, smoothing vertices of degree two except if this introduces parallel edges and one that removes all vertices not contained in any cycle. The next picture presents some of the results obtained with this tool. 


We believe that due to the large thickness of the input image, the final network is not good as expected. Decreasing thickness on the input image (this means having only pure triangles) the final network appears as completely disconnected, laying our solver with better performance.




==> sections/Notation.tex <==
An \textit{unweighted graph}  $G$ is a pair $(V_G,E_G)$ of vertices $V_G$ and edges $E_G$ (a set of subsets of $\{\{v,w\}:v,w\in V\}$), sometimes simply called a graph. We use the subscript $\cdot _G$ to reference the graph $G$, but sometimes we simply use $V$ and $E$ without the subscripts. When dealing with many graphs, we would omit the indexation and we will use $V(G)$ (or $E(G)$) to reference \textit{the set of vertices of $G$ (or $E(G)$}.) 

%\DLcom{ An \textit{unweighted graph} $G$ (or simply a \textit{graph}) is a pair $G = (V_G, E_G)$ of vertices $V_G$ and edges $E_G$, set of subsets of $\{\{v,w\}:v,w\in V\}$. Here, we use the subscript $\cdot _G$ to reference a graph $G$, or simply $V$ and $E$ (without the subscripts). When dealing with many graphs, we omit the indexation and use $V(G)$ (or $E(G)$) to reference \textit{the set of vertices of $G$ (or $E(G)$}.)}

A \textit{weighted graph} $G$ is a triplet $(V_G,E_G,w_G)$ of vertices $V_G$, a set of edges $E_G$ (a set of subsets of $\{\{v,w\}:v,w\in V\}$) and a function $w_G:A\rightarrow B$, where $A\in \{V_G,E_G\}$ and $B$ is any set (usually, $B\in \{\mathbb{R}^+,\mathbb{R}^2\}$) . For each $x\in A$, the value $w_G(x)$ is called the \textit{weight} of $x$.  The previous comments about the notation for unweighted graphs also apply to these ones. The \textit{unweighted version} of a weighted graph $(V_G,E_G,w_G)$ is the pair $(V_G,E_G)$.



%%%%\DLcom{A \textit{weighted graph} $G$ is a triplet $G = (V_G,E_G,w_G)$, with vertices $V_G$, a set of edges $E_G$ (a set of subsets of $\{\{v,w\}:v,w\in V\}$) and a function $w_G:A\rightarrow \mathbb{R}^+$, where $A\in \{V_G,E_G\}$ . For each $x\in A$, the value $w_G(x)$ is called the \textit{weight} of $x$.  The previous comments about the notation for unweighted graphs also apply to these ones. }

When the set of edges $E_G$ is a subset of $\{\{v,w\}:v,w\in V\}$, we say that the graph is \textit{undirected}. If $E_G\subset \{(v,w):v,w\in V_G\}=V_G^2$, then we say that the graph $G$ is \textit{directed}. The previous definitions were given for undirected graphs, but they also apply for directed graphs. For each edge $e\in E_G$, there exist $v,w\in V_G$, such that $e=(v,w)$; the node $v$ is called the \textit{origin} of $e$ and $w$ is called the \textit{end} (or \textit{tail}) of $e$.   An arrow pointing from $v$ to $w$ is the standard way of representing directed edges.

If more than one \textit{weight} function $w_G$ needs to be defined for a particular unweighted graph $G$, then we specify them as elements in a tuple together with $G$, i.e., let $n\geq 1$ and $f_1, f_2, ..., f_n:A\to B$ be  weight functions for an unweighted graph $G=(V_G,E_G)$ where $A\in \{V_G,E_G\}$, then we redefine $G$ as the tuple $(V_G,E_G, f_!,f_2, ...,f_n)$. A graph $G=(V,E,f_1,f_2,...,f_n)$ is called a \textit{multi-weighted} graph.   

A \textit{subgraph} $H=(V_H,E_H)$ of a graph $G=(V_G,E_G)$ is a graph s.t., $V_H\subset V_G$ and $E_H\subset E_G$. For weighted graphs $G=(V_G,E_G,f)$, a \textit{weighted subgraph} is a graph $H=(V_H, E_H,f_H)$ where $(V_H,E_H)$ of the unweighted version of $G$ s.t., $f_H:=f\restriction_{A},$ where $A\in \{ V_G,E_G\}$. The symbol $g\rectriction_B$ denotes the restriction of the function $g$ to the set $B$.    

==> sections/basis_pursuit_intro.tex <==
% !TEX program = pdflatex
% !TEX root = many .tex files

\subsection{Basis Pursuit}\label{basis_pursuit_section}

Let $G$ be a directed graph with $n$ nodes and $m$ edges. Write
\begin{align*}
V(G)&=\{v_1,v_2,...,v_n\}, \\
E(G)&=\{e_1,e_2,...,e_m\}.
  \end{align*}



  The \textit{incidence matrix} $A$ of the graph $G$ is a $n\times m$ matrix such that its entry $ij$ is defined as
  $$
  [A]_{ij}=\left\{
\begin{array}{lcl}
      & 1, & \text{ if } e_j=(v_i,x) \text{ for some }x\in V(G),\\
      -& 1, & \text{ if }  e_j=(x,v_i) \text{ for some }x\in V(G),\\
      & 0, & \text{ other cases} 
\end{array} 
\right.
  $$
for all $i\in \{1,...,n\}, \ j\in\{1,..,m\}.$ Note that for a fixed index $i$, it is true that 

$$
\text{deg}_{-}(v_i)=\!\!\sum_{j,[A]_{ij}>0} [A]_{ij} \ \text{ and } \
\text{deg}_{+}(v_i)=-\!\!\sum_{j,[A]_{ij}<0} [A]_{ij}, 
$$
where $\text{deg}_{-}(v_i),\text{deg}_{+}(v_i)$ represent the outer and inner degree of the node $v_i$,  respectively. 

For instance, the incidence matrix $A$ of the graph $G$ in Figure \ref{incid} is


\begin{align*}
\begin{array}{cccccc}
\ \ \ e_1 \  & \  e_2 \  & \ \ e_3 \  & \ \ e_4 \  & \ \ e_5 \  & \ \ e_6 \ \ \ 
\end{array} \\
\left(
\begin{array}{cccccc}
 1 & 1 & 1 & 0 & 0 & 0\\
-1 & 0 & 0 & 1 & 0 & 0 \\
0 & -1 & 0 & 0 & 1 & 0 \\
0 & 0 & -1 & 0 & 0 & 1 \\
0 & 0 & 0 & -1 & -1 & -1
\end{array} 
\right)
\end{align*}


\begin{figure}[h]
\centering
\includegraphics[scale=0.3]{figs/graph_incidence.png}
\caption{Directed graph $G$}\label{incid}
\end{figure}


Imagine now that we want to add some weights to the nodes in $G$ using a function $f$ defined explicitly in the following way:
$$
\begin{array}{cccc}
f(v_1)&=& &1, \\
f(v_2)&=& &0, \\
f(v_3)&=& &0, \\
f(v_4)&=& &0, \\
f(v_5)&=&-&1
\end{array} 
$$
These values could represent the flow of water that each node is receiving, coming from external sources. Positive values correspond to in-coming flow and negative values to out-going flow. 0-flow means neither injection or extraction. Figure \ref{incid_ss}  shows a representation of this situation. From now on,  vertices $v\in V$ are called \textit{sources} (\textit{sinks})  if they satisfied the condition $f(v)>0$ ($f(v)<0$).



\begin{figure}[h]
\centering
\includegraphics[scale=0.32]{figs/graph_sources_sinks.png}
\caption{Sources and sinks in $G$}\label{incid_ss}
\end{figure}

We represent the \textit{external sources} as new links. Essentially, we could see $G$ as a system of tubes (represented by the edges) with different injection points (represented by the nodes), in which 1 unit of water flows. In this framework, can we say what is the amount of water flowing between different nodes?

In order to give an answer to this question, we could solve the following system of equations:

$$
\begin{array}{cccccc}
\overbrace{\ \ \ \ \ \ f(v_1)\ \ \ \ \  }^{injection}&-&\overbrace{(x_1+x_2+x_3)}^{extraction} & + &\overbrace{\ \ 0 \ \ }^{0-flow} &=0   \\
x_1&-&x_4&+& f(v_2)&=0, \\
x_3&-&x_6&+&f(v_3) &=0, \\
x_2&-&x_5&+&f(v_4) &=0, \\
x_4+x_5+x_6&-&f(v_5)& & &=0
\end{array}, 
$$
that can be re written in a matrix way $A \ \mathbf{x} = \ \mathbf{b}$, where $A$ is the incidence matrix showed before and  $\mathbf{b}\in \mathbb{R}^{n}$ is defined as $[\mathbf{b}]_i=f(v_i),$  $\forall i \in \{1,...,n\}$.

A very intuitive solution of this system is shown in Figure \ref{incid_flow}. Other solutions can be found by adding more flow to one of the edges $e_1,e_2$ or $e_3$, and then doing the corresponding substractions to keep it balanced. 

\begin{center}
\includegraphics[scale=0.32]{figs/graph_flow.png}
\begin{figure}[!h]
\caption{Flow distribution in $G$}\label{incid_flow}
\end{figure}
\end{center}

An interesting way of thinking about the flow problem is attained if we add some cost contrains. Let's start with an easy case, imagine that each unit of edge length can transport at most 1 unit of water and it has an associated fixed cost $c\in \mathbb{R}$. Thus, if an edge $e$ has length equal to 1, and we decide to send some water flow through it, the cost of this task will be equal to $c$. In this new framework, our goal of finding a distribution of flow for our system of tubes can be recasted as a design problem: Build a network $G'$, such that $V(G')=V(G),$ $A_G=A_{G'}$ and find $\mathbf{x}$, such that 
$$
A_{G'} \mathbf{x} = \mathbf{b},
$$
where $\mathbf{b}$ is the extraction/injection vector and $x$ contains all the information about the lengths of the edges of $G'$ (which also is the flow distribution of the system!). Once that a solution $\mathbf{x}$ is found, we can compute the total cost of our flow distribution in the following way:
$$
cost(\mathbf{x})=c\cdot\sum_j \ [\mathbf{x}]_j.
$$

For instance, the total cost for the flow distribution shown in Figure \ref{incid_flow} is $2c$. This case of constant cost $c$ and unitary length for all the edges is a very trivial one. In fact, it is easy to prove that 
$$
cost(\mathbf{y})=\sum_{i,f(v_i)>0} f(v_i) -\sum_{i,f(v_i)<0} f(v_i), \ \ \ \forall \mathbf{y}\in \mathbb{R}^n,
$$
which is independent of $\mathbf{y}$, and thus, optimization is not possible. Real problems appear for costs depending on the edges. The difficulty of solving them could increase until the point in which no solutions exist.  This wider family of minimization problems is known as Transportation Problems (ref ? examples). 

A less restrictive problem related to the previous discussion (and very relevant to  it!) is the one known as the \textit{Basis Pursuit}, which can be stated formally in a very general way as follow:

\textbf{Basis Pursuit Problem:}


Let $A$ be a matrix in $\mathbb{R}^{n\times m}$ and $\mathbf{b}$ a vector in $ \mathbb{R}^m$, find $\mathbf{x}\in \mathbb{R}^n $ such that 
$$
\mathbf{x}\in \underset{\mathbf{y}\in \mathbb{R}^n }{\text{arg min}} \sum_j \ |[\mathbf{y}]_j| \ \ \ \text{subject to} \ \  A \ \mathbf{x} = \mathbf{b}.
$$
The minimization function shown before is the $l_1$ \textit{norm} of the vector $\mathbf{y}$, denoted as $|| \mathbf{y}||_1$.  The problem can be restated as

$$
\text{find} \ \ \mathbf{x}\in \mathbb{R}^n \ \ \text{such that} \ \ \mathbf{x}\in \underset{\mathbf{y}\in \mathbb{R}^n }{\text{arg min}} \ || \mathbf{y}||_1  \ \ \ \text{subject to} \ \  A \ \mathbf{x} = \mathbf{b}.
$$

A graph-adapted BP problem can be stated in the following way:

\textbf{Graphic Basis Pursuit (or \textit{Optimal Transshipment}) Problem :}


Let $G=(V,E,w)$ be a weighted graph. Suppose that $G$ consists of $n$ vertices and $m$ edges. Assume that $E=\{e_1,...,e_m\}$.  Let $A$ be the incidence matrix of $G$. 


For a given $\mathbf{b}$ in $ \mathbb{R}^m$, find $\mathbf{x}\in \mathbb{R}^n $ such that 
$$
\mathbf{x}\in \underset{\mathbf{y}\in \mathbb{R}^n }{\text{arg min}} \sum_j \ |[\mathbf{y}]_j| w(e_j) \ \ \ \text{subject to} \ \  A \ \mathbf{x} = \mathbf{b}.
$$

Now the goal is to minimize a weighted $l_1$ norm of the vector $y$, denoted as $||\mathbf{y}||_{1,w}$. It can be restated as 

$$
\text{find} \ \ \mathbf{x}\in \mathbb{R}^n \ \ \text{such that} \ \ \mathbf{x}\in \underset{\mathbf{y}\in \mathbb{R}^n }{\text{arg min}} \ || \mathbf{y}||_{1,w}  \ \ \ \text{subject to} \ \  A \ \mathbf{x} = \mathbf{b}.
$$

Note that the case of unitary weights (i.e. $w(e)=1,  \ \forall e$) takes us back to the $l_1$ optimization problem.  

As we showed in the beginning of this section, this problem could be thought as a flow problem (even though, no flow constraints are showed) where the structure of the system is given by the graph $G$, the source and sink configuration is described by $\mathbf{b}$ and the distribution of the optimal flow is contained in the vector $\mathbf{x}$.  Note that in the case where $w(\cdot)$ is the length function, the cost of sending $[\mathbf{x}]_j$ through the edge $e_j$ is proportional to the length of the edge $e_j$. Thus, avoiding large flows in long edges could lead to lower overall costs. 

The reason why we motivated these problems as flow distribution tasks is  that they happen to be highly related to the behaviour of the \textit{Physarum Polycephalum} (PP) and the flow of food inside its body parts. The PP Dynamical problem stated in section \ref{ppd} can be rewritten in terms of matrices as follows: 

Given a graph $G=(V,E,w)$ with $n$ vertices $\{v_1,v_2,...,v_n\}$ and $m$ edges $\{e_1,e_2,...,e_m\}$, $A$ its incidence matrix, and $f:V\rightarrow \mathbb{R}$ such that
$$
\sum_{v\in V} f(v)=0,
$$ 
find $\boldsymbol{\mu}: [0,\infty)\rightarrow \mathbb{R}^m$ and $\mathbf{u}: [0,\infty)\rightarrow \mathbb{R}^n$ solving the system of equations 

\begin{equation}\label{PPdyn}
\begin{array}{rl}
\textbf{q}(t)=&\text{diag}(\boldsymbol{\mu}(t)) \ \text{diag}(\mathbf{w})^{-1} \ \mathbf{A}^{T} \ \mathbf{u}(t) \ , \\
\mathbf{A} \ \mathbf{q}(t) =& \mathbf{f} \ , \\ 
\boldsymbol{\mu}'(t)=&| \ \mathbf{q}(t) \ |-\boldsymbol{\mu}(t) \ ,\\
\boldsymbol{\mu} (0)>&0
\end{array}
\end{equation}


where $|\cdot|$ represents the absolute value computed component-wise. For each $1\leq i\leq n$, the value $[\boldsymbol{\mu}(t)]_i$ corresponds to the \textit{potential} at the node $v_i$ at time $t$. For each $1\leq i\leq m$, the values $[\boldsymbol{u}(t)]_j$ and $[\boldsymbol{q}(t)]_j$  correspond to the \textit{conductance} and the \textit{flow} resp., of the edge $e_j$ at time $t$.  In \cite{bonifaci2012physarum} it was proved that vector $\mathbf{q}(t)$ converges to a steady state $\mathbf{q}^*\in \mathbb{R}^m$, as $t\rightarrow \infty$, and this $\mathbf{q}^*$ is  a solution of the Graphic BP problem. 

As we know the PP Dynamical problem also inspired the  DMK. In the next section we show how the approach used to solve the DMK equation can be used to obtain solutions the Graphic BP problem.

\subsection{BP problem solved using the DMK approach}\label{BP_thru_DMK}

As we mentioned before it is well-known that solving PP Dynamical problem will lead to the solution of the BP problem. Therefore, adaptations of the DMK solver to the PP Dynamical are a reasonable starting point for us when looking for solutions of the Graphic BP. 

Let's start by recalling the DMK problem stated in section \ref{dmkSection}. Consider a convex, bounded a smooth domain $\Omega\subset \mathbb{R}^d,$ a function $f\in L^2(\Omega)$ with $\int_\Omega f = 0,$ and a strictly positive function $\mu_0$ on $\Omega.$ Find $u:[0,\infty)\times \Omega \rightarrow \mathbb{R}$ and $\mu:[0,\infty)\times \Omega \rightarrow \mathbb{R}$ solving 

\begin{equation}\label{DMK}
\begin{array}{rl}
&-\text{div}(\mu \nabla u) = f, \\
&\partial_t (\mu ) = |\mu\nabla u|- \mu, \\
&\mu(0,x)=\mu_0(x),
\end{array}
\end{equation}

where the first equation is intended in a weak sense. Another requirement for the first equation is to impose zero Neuman Boundary conditions, meaning that the derivatives of $\mu$ and $u$ are equal to zero at $\partial \Omega$.

Note now that the PP Dynamical problem can be rewritten in the following way:

Define 
$$
\nabla := \text{diag}(\mathbf{w})^{-1}\mathbf{A}^T, \ \ \ S[\mu(t)]:= \mathbf{A} \ \text{diag}(\mu (t)) \ \text{diag}(\mathbf{w})^{-1} \ \mathbf{A}^T, \ \ \ C[\mu]:=\text{diag} (\mu(t)),
$$

and replace them in eq., \ref{PPdyn} to get

\begin{equation}\label{newDMK}
\begin{array}{rcl}
S[\mu(t)] \ u(t) &=& \mathbf{f} \ , \\ 
\mu'(t)&=&|\mathbf{q}(t)|-\mu(t) \ \\
	   &=& |C[\mu(t)] \ \text{diag}(\mathbf{w})^{-1} \ \mathbf{A}^{T}u(t)|-\mu(t)\\
	   &=& |C[\mu(t)] \ \nabla u(t)|-\mu(t),\\
\mu (0)&>&0,
\end{array}
\end{equation}

which is similar to DMK problem (eq., \ref{DMK}).

Discretization of equation \ref{newDMK} by the implicit backward Euler scheme leads to the following sequence of nonlinear algebraic equations for $(u^{k+1},\mu^{k+1})$:

\begin{equation}\label{implicit}
\begin{array}{rcl}
S[\mu^{k+1}] \ u^{k+1} &=& \mathbf{f} \ , \\ 
\dfrac{\mu^{k+1}-\mu^{k}}{\Delta t_k}&=&C[\mu^{k+1}] \ |\nabla u^{k+1}|-\mu^{k+1}.
\end{array}
\end{equation}

The previous constructions show that we can apply the same scheme applied for DMK to solve equations, and once that it is solved, solutions for Graphic BP are found. From now on, this way of solving the PP Dynamical problem will be called \textit{discrete} DMK solver. We omit the details about the Newton method applied to solve equation \ref{implicit}. The complete scheme is explained  in \cite{facca2016towards}. 



%%% Local Variables:
%%% mode: latex
%%% TeX-master: 
%%% End:


==> sections/bp_vs_steiner.tex <==
% !TEX program = pdflatex
% !TEX root = many .tex files

\subsubsection{BP simplification as a filtering candidate}\label{bp_filtering}

Let $G$ be a weighted graph, $A$ its incidence matrix, $f$ be a source-sink distribution and assume that $\mathbf{x^*}$ is one solution (obtained with the discrete DMK solver) of the Graphic BP problem associated to $G$ and $f$, i..e, 

\begin{equation}\label{solution}
|| \mathbf{x}^*||_{1,w}\ = \ \underset{\mathbf{y}\in \mathbb{R}^n }{\text{min}} \ || \mathbf{y}||_{1,w}  \ \ \ \text{subject to} \ \  A \ \mathbf{x}^* = \mathbf{f}
\end{equation}

Thus, $\mathbf{x}$ contains information about the optimal distribution of flow in the graph $G$. But, can we say something \textbf{\textit{else}} about the optimality of $\mathbf{x}$ apart from \ref{solution}? 

To give an answer to this question, we need to come back to the PP Dynamical problem. Remember that $\mathbf{x}^*$ is the \textit{limit} as $k$ goes to $\infty$ of a sequence $\{\mathbf{x}^k\}_k$ given by 

\begin{equation}\label{qeq}
\mathbf{x}^k =\text{diag}(\mu^k) \ \text{diag}(\mathbf{w})^{-1} \ \mathbf{A}^{T} \ \mathbf{u}^k
\end{equation}

where the sequences $\{\mu^k\}_k$ and $\{ u^k\}_k$ are the ones obtained using the discrete DMK solver. This means that for each one of the pairs $\mu^k$ and $u^k$, we can think about having a new graph 
$$
G^k:=(V(G),E(G),w_k)
$$

where $w_k(e):=\mathbf{x}^k(e), \ \forall e\in E(G)$, and $\mathbf{x}^k$ is computed using the equation \ref{qeq}.


According to \cite{bonifaci2012physarum}, the sequence $\{\mathbf{x}^k\}_k$ converges to a steady state that contains the information about the shortest path connecting sources and sinks.
This means that the sequence of graphs $\{G_k\}_k$ \textit{converges} to a graph path $S$, with minimal total length. But, isn't $S$ of the form $(V(G),E(G),w)$ for a $w$ obtained as a limit? How is it possible that the set $E(G)$ degenerates to a path? The answer to this question is given by the fact that for $k$ big enough, there exist a set $E'\subset E(G)$ such that 
$$
0\leq w(e)\ll 1, \ \ \forall e\in E'.
$$   

Therefore, if we \textit{remove} all the edges $e\in E'$ from $E(G)$ and the isolated vertices obtained once that these edges are removed, we get a subgraph of $G$ that is a path graph ($S$). So, in simple words, $S$ is the subgraph of $G$ consisting of the nodes that have a significant amount of flow. Note that the steady state of the PP dynamics showed before is $\mathbf{x}^*$, our solution to the Graphic BP problem.  Thus, solutions of the Graphic BP problem tell us weighted shortest\footnote{The adjective "weighted shortest" is given in the sense of minimizing the norm $||\cdot ||_{1,w}$} ways of transporting resources from senders to receivers.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: 
%%% End:


==> sections/delaunay_voronoi_intro.tex <==
% !TEX program = pdflatex
% !TEX root = many .tex files

%\section{Delaunay Triangulations and Voronoi Sets}

A \textit{Delaunay triangulation} for a given set $\mathcal{P}$ of $N$ points in $\mathbb{R}^2$ is a triangulation $DT(\mathcal{P})$ such that no point in $\mathcal{P}$ is inside the circumcircle\footnote{The \textit{circumcircle} is a circle that passes through all the points.} of any triangle in $DT(\mathcal{P})$. For instance, if $\mathcal{P}$ is the set of points showed in Figure \ref{delaunay1}, then the triangulation showed in the same plot is a Delaunay triangulation. Note that for any three points in $\mathcal{P}$, the gray circle (the circumcircle) does not contain any other point in $\mathcal{P}$ (not all the circumcircles are shown, but it is indeed a \textit{DT}).

 
\begin{center}
\includegraphics[scale=0.15]{figs/delaunay1.png}
\label{delaunay1}
\begin{figure}[!h]
\caption{Example of a Delaunay triangulation}
\end{figure}
\end{center}
 
 Note that if a set of points generates a triangulation in which each triangle is equilateral, then this triangulation must be $DT$. Thus, sets which consist of points that are \textit{uniformly distributed} in the plane are more likely of generating Delauney triangulations.  
 
 
For any triangle, its circumcenter\footnote{The \textit{circumcenter} is the center of the circumcircle} can be computed as the intersection of the three bisectors of their sides. A natural graph representation of a triangulation can be obtained by joining the circumcenters of the triangles that share a side.  When this is done for a Delaunay Triangulation of a set $\mathcal{P}$, the result is called the \textit{dual graph} of the \textit{Voronoi diagram} of $\mathcal{P}$. \textit{Dual graphs} are the graphs obtained from a particular planar graph $G$ by placing a node on each one of the faces of $G$ (Figure \ref{dg} shows an example of a dual graph). 

\begin{center}
\includegraphics[scale=0.15]{figs/dualgraph.png}
\label{dg}
\begin{figure}[!h]
\caption{A graph $G$ ({\color{blue}blue}) and its dual ({\color{red}red}).}
\end{figure}
\end{center}

The definition of a Voronoi diagram is slighty more difficult to state so for the moment we will use the definition of the dual graph of the Voronoi diagram to define an intuitive notion of the actual definition: The Voronoi set associated to a Delaunay triangulation of a set $\mathcal{P}$ is a partition of the plane given by the set of faces of the dual graph of the Voronoi diagram of DT. For the example given in the Figure \ref{dg}, the Voronoi set would be the partition of the plane given by the graph in red. Voronei diagrams can be introduced without the notion of Delaunay triangulations. The actual definition will be presented later on.


An example of the dual graph of the Voronei Diagram is showed in the Figure \ref{voronoi1}. It was build from the Delaunay triangulation showed in Figure \ref{delaunay1}. 

\begin{center}
\includegraphics[scale=0.15]{figs/voronoi1.png}
\label{voronoi1}
\begin{figure}[!h]
\caption{Dual graph (red) of the Voronoi set of a Delaunay triangulation (black)}
\end{figure}
\end{center}

A first interesting property about the Voronoi diagrams is that if they are built from Delaunay triangulations, then all of its sets are convex, even the unbound ones ({\color{red} FALSE! Check \href{http://www-cs.ccny.cuny.edu/~wolberg/capstone/voronoi/voronoiSurvey.pdf}{Vornoi Diagrams - A Survey of a Fundamental Geometric Data Structure} Why using Delaunay triangulations then?}.

The next subsection shows a deeper analysis of Voronoi diagrams. 

\subsection{Defining Voronoi diagrams}

The definition of the dual graph of the Voronoi diagrams is very intuitive when looked from the perspective of Delaunay triangulations. But what is a Voronoi diagrams? and why we use Delanuy triangulations to define them?

Let's answer formally the first question:  



\subsection{Optimal networks as dual graphs of Voronei diagrams}

As it has been mentioned before, we are interested in getting a \textit{robust-enough} graph representation of the solution of different Monge-Kantorovich problems that are related to Optimal Transportation settings. In this section we present a basic idea about a representation of these solutions given by Voronoi diagrams. 

Let's recap that the DMK problem we are interested in is described by the following equations 
\begin{subequations}\label{eq:2}
    \begin{align}
&-\text{div}\left( \mu (t,x) \nabla u(t,x)\right)=f^+(x)-f^-(x)\\
         &\partial_t \mu(t,x)=\left(\mu(t,x)\nabla u(t,x)\right)^\beta-k(x)d(t)\mu^\alpha(t,x)\\
         &\mu(0,x)=:\mu_0(x)>0      
  \end{align}
\end{subequations}

In order to solve this, Facca and Putti use Finite Element Methods through a discretization of both space and time on a double level grid. Finding a solution for the system \ref{eq:2} is the same as finding a potential and a conductance for all of the different triangles in the grid. The way they solve this is by using the relation

\subsection{voronoi cells to community detection}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: 
%%% End:


==> sections/dmk_model.tex <==
% !TEX program = pdflatex
% !TEX root = ../main.tex


\paragraph{Continuos representation: the dynamical Monge-Kantorovich problem}\label{dmkSection}

An analogous version of the problem described in \cite{bonifaci2012physarum} for a continuous domain like an open and bounded subset $\Omega$ of $\mathbb{R}^2$, was proposed by \cite{facca2016towards}:

Consider the system of partial differential equations:
\begin{subequations}\label{eq:2}
    \begin{align}
&-\text{div}\left( \mu (t,x) \nabla u(t,x)\right)=f^+(x)-f^-(x)\\
         &\partial_t \mu(t,x)=\left(\mu(t,x)\nabla u(t,x)\right)^\beta-k(x)d(t)\mu^\alpha(t,x)\\
         &\mu(0,x)=:\mu_0(x)>0
  \end{align}
\end{subequations}

complemented by zero Neumann boundary conditions. In this scenario, the problem consists in finding a pair of functions $(\mu, u ):[0,+\infty)\times \Omega\rightarrow \mathbb{R}^+\times \mathbb{R}$ that satisfies the  DMK Equations.  %It receives the Monge-Kantorovich name because it can be proved that it is equivalent to the classical problems of optimal transportation theory stated by Monge (\cite{villani2008optimal}, p.22) and a few years later restated by Kantorovich (\cite{villani2008optimal}, p.22). 
It was shown that finding the pair $(\mu, u )$ is equivalent, under certain conditions, to find a mapping $\gamma$ that turns one measure $\mu^+$ into another measure $\mu^-$ minimizing a given cost function $c$.

The authors \cite{facca2016towards} proposed, among other things, an algorithm for solving the weak formulation of the double discretization in time and space of the system  \ref{eq:2}.  They showed that this solver (or \textit{DMK solver}, from now on) was also able to emulate the results found by \cite{tero2007mathematical} for the discrete formulation (PPD problem). By tuning some parameters of the equations like the exponent $\beta$, they were able not only to model different problems belonging to the optimal transportation theory but also to solve them using their mentioned tools. A brief description of the formulation used to solve this problem is given in Section \ref{BP_thru_DMK}.

Each time that the solver is executed, we find a sequence of functions $(\mu_t,u_t)_t$ defined on each one of the elements of the grid, the first one representing  the transport density ($\mu_t$) at time $t$ and the second one representing the potential $u_t$, at a given time $t$. If this sequence converges, then its limit is denoted as $(\mu^*, u^*)$. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: ''main.tex''
%%% End:


==> sections/find_terminals.tex <==
% !TEX program = pdflatex
% !TEX root = main.tex

\subsubsection{How to compute the \textit{terminals}?}\label{terminals}

In order to get the set $T\subset V$ of \textit{terminals}, we implemented three different criteria based on \textit{betweenness centrality, degree centrality} and \textit{directed graphs.} 

\textbf{Betweenness centrality:}
First, we build from $G=(V,E,w,p)$, the node-weighted graph $G'=(V,E,\text{bc})$ using the betweenness centrality of the nodes in $G$ (see Section \ref{betweenness_centrality}). Once this is done, we define $T_{a,b}$ as
$$
T_{a,b}:=\{v\in V: \text{bc}(v)\in [a,b]\}
$$
where $a:=\underset{v\in V}{\min} \ \text{bc}(v)$, $b:=a\cdot \gamma,$ and $\gamma\in [1,c]$ for $c=\underset{v\in V}{\max} \ \text{bc}(v)$ is a control parameter.  If $\gamma=1,$ we define $T$ as the set of nodes with minimal betweenness centrality.  If $\gamma= c,$ then $T_{a,b}=V.$ 


\textbf{Degree centrality:} We define $T_\alpha$ as
$$
T_\alpha:=\{v\in V: \text{deg}(v)=\alpha\},
$$
where $\alpha=\underset{v\in V}{\min} \ \text{deg}(v)$. If $\alpha=1,$ then $T$ is the set of leaves of $G$. 

\textbf{Directed graph:} We build a weighted directed graph $G_d=(V_{d},E_{d},p_d)$ from $G$, where $V_d$ is the set of vertices of $V$ and $p_d(v)$ gives the location $(x_v,y_v)$ of the vector $v$ in the set $\Omega$. The set of edges is defined from $E$ in the following way: Let $e=\{u,w\}\in E$, $p_d(u)=(x_u,y_u),$ $p_d(w)=(w_x,w_y)$. If $x_u<x_w,$ then add the edge $(u,w)$ to the set $E_d;$ otherwise, add the edge $(w,u)$.

We define the \textit{set of out-flow nodes} $T^+$ and the \textit{set of in-flow nodes} $T^-$ as 
$$
\begin{array}{rl}
T^+:=&\{v\in V_d: \text{deg}^+(v)>0, \text{deg}^-(v)=0\}, \\
T^-:=&\{v\in V_d: \text{deg}^-(v)>0, \text{deg}^+(v)=0 \},
\end{array}
$$
 where $\text{deg}^+(v)$ is the \textit{out-degree} of $v$ and $\text{deg}^-(v)$ is the \textit{in-degree} of $v$. Then, the set of \textit{terminals} is $T:=T^+\cup T^-.$

This way of defining $G_d$ was intended to use the edges to represent the direction of the flow from source to sink, in general. It fails in some particular situations, and the improvement of this algorithm is part of our future plans.   





%VisIt is a free interactive parallel visualization and graphical analysis tool for viewing scientific data. Users can generate visualizations from their data, animate them through time, manipulate them, and save the resulting images for presentations. It also contains a rich set of visualization features so that you can view your data in a variety of ways. It can be used to visualize scalar and vector fields defined on two- and three-dimensional (2D and 3D) structured and unstructured meshes. 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> sections/implementation_graph_extraction_1.tex <==
% !TEX program = pdflatex
% !TEX root =  ../main.tex

------------------------------------------------------------------------------------------------------------------------\\
\CDBcom{This all section will go into the readme.md file on the github}
\subsection*{Implementation}
We provide now a pseudo-code corresponding to the \textit{graph extraction} step which outputs a \textit{python}-friendly network structure. The details about this algorithm and all the subroutines are explained below. We write in italic the subroutines. 

The input files are:
\begin{itemize}
\item \textit{opt\_tdens.dat}: these are the optimal values of the transport density for each one of the barycenters of the grid. 
\item \textit{graph\_cell.dat}: The positions of the nodes of the graph generated by the DMK solver. The links of this graph. 
\item \textit{grid.dat}:  it contains the positions of the nodes and the edges of the grid.
\item A threshold $\tau \in [0,1]$:   it represents a percentage of maximum transport density, i.e., $\delta=\tau \times W $, where $W$ is the maximum transport density and $\delta$ is the one shown in Section \ref{theory_for_graph_extraction_implem}.
\item \textit{graph\_type:} this is a flag for the type of graph the user wants to get as output. It could be either 1 (Section \ref{theory_for_graph_extraction_implem}), 2 (Section \ref{graph2}) or 3 (Section \ref{graph3}). 
\end{itemize}

\textbf{Algorithm:} Graph Extraction.     

\textbf{Input:} opt\_tdens.dat, graph\_cell.dat, grid.dat, a threshold $\tau$, graph\_type.
    
\textbf{Output:} A weighted graph $G$ (if \textit{graph\_type}$!=$ 3,  $G:=(V_G,E_G,w,p)$; if not, $G:=(V_G,E_G,p)$). The function $w$ represents the optimal transport density $\mu$ as explained in Section \ref{theory_for_graph_extraction_implem}. The function $p$ maps each vertex $v\in V$ into a duple $(x_v,y_v)\in \mathbb{R}^2$ representing the position of $v$ in the domain $\Omega$.
  

\begin{enumerate}
\item Get the positions of the barycenters (\textit{get\_bary}) and store them as values of a dictionary \textbf{D} (\textit{bar2dict}).  The keys of this dictionary are given by the positions in the files of such barycenters. For instance, if the barycenter $(x,y)$ appears in the $\text{10}^{th}$ line in the list, then we define $\text{\textbf{D}}[\text{10}]=(x,y)$.
\item Read the weights from the dat file (\textit{extracting\_weights}) and saving them in a dictionary \textbf{W} (\textit{weight2dict}).
\item Compute the maximum weight $W$.
\item Read the grid.dat file as a list.
\item Reconstruct the grid used to solve the DMK equations: first, as a dictionary, then, as a graph $G_\Delta=(V_{G_\Delta}, E_{G_\Delta},q_{G_\Delta})$. $q_{G_\Delta}$ is a node weight function mapping each node to its position in the domain.
\item Define $p$:
\begin{enumerate}
\item If \textit{graph\_type}$!=$ 3, add the keys of \textbf{D} as nodes of a graph $G$. Define the function $p$ as $p(v):=\text{\textbf{D}}[v], \ \forall v$ in the keys of \textbf{D}.
\item If \textit{graph\_type}$=$ 3, define $V_G:=V_{G_\Delta}$ and $p(v):=q_{G_\Delta}(v), \ \forall v\in V_G$. 
\end{enumerate}
\item For each node $v$ in $G$, look for the triangle $\Delta_v$(informally, in $G_{\Delta}$) such that $v$ is its barycenter (\textit{get\_first\_neig}). The nodes $V(\Delta_v)$ are called \textit{first neighbours} of $v$.

\item For each node $v$ in $G$, 
\begin{enumerate}
\item If \textit{graph\_type} $=$ 3, test the condition:
$$
\text{\textbf{W}}(v)\geq\delta.
$$
If it is true, add $V(\Delta_v)$ to $V(G)$ and $E(\Delta_v)$ to $E(G)$.

\item If \textit{graph\_type} $!=$ 3, look for all the triangles that share:
\begin{enumerate}
    \item either an edge (if \textit{graph\_type} $=$ 2)
    \item or a node (if \textit{graph\_type} $=$ 1)

 with the triangle $\Delta_v$ (\textit{get\_sec\_neig}). All these triangles are called \textit{second neighbours} of $v$. Suppose that $n$ is the number of second neighbours of $v$. Denote them as $\{\Delta_v^i\}_{i=1}^n$.

\item  For each $\Delta_v^i$, detect its barycenter $\overline{v}^i$, and then test the condition:
$$
\text{\textbf{W}}(v) \geq \delta, \ \text{and} \ \ \text{\textbf{W}}(\overline{v}^i) \geq \delta .
$$
If it is true, add the edge $e^i=\{v,\overline{v}^i\}$ to the set of edges $E$ of $G$, and define $w(e^i)=\min \{\text{\textbf{W}}(v),\text{\textbf{W}}(\overline{v}^i)\}$. This is explained in the item 4 of the algorithm in Section \ref{theory_for_graph_extraction_implem}.

\end{enumerate}
\end{enumerate}
\item Remove of $G$ the set of vertices
$$
\{ u \in G: \text{deg}(u)=0\}.
$$
\item Return $G$.
\end{enumerate}

Note that if \textit{graph\_type} $!=$ 3, the only information used from the file \textit{graph\_cell.dat} is the one corresponding to the locations of the nodes. Links between nodes are defined later on in the algorithm. 

Step 7 of the algorithm is necessary to obtain all the second neighbors of each barycenter. Let $v$ be the barycenter of a triangle $\Delta_v,$ whose vertices are  $w_1,w_2,w_3$. In order to find the second neighbors of $v$, we ask about the membership of its first neighbours to all the different triangles  $\Delta_v^*\in G_\Delta$: to get the triangles $\Delta_v^*$ that share an edge with $\Delta_v$, the Boolean vector $b_{w_1,w_2,w_3}=[w_1\in \Delta_v^*, w_2\in \Delta_v^*, w_3 \in\Delta_v^*]$  has to contain exactly two \textbf{True} values. To get the triangles $\Delta_v^*$ that share a node with $\Delta_v$, the vector $b_{w_1,w_2,w_3}$ has to contain exactly one \textbf{True} value. 
------------------------------------------------------------------------------------------------------------------------\\
%%% Local Variables:
%%% mode: latex
%%% TeX-master: 
%%% End:


==> sections/other_graph_extractions_1.tex <==
% !TEX program = pdflatex
% !TEX root = ../main.tex 

%\section{The model}

\paragraph{Using only side links}
%The second  proposed way of constructing the graphs that we mentioned before is the following one.  

\begin{enumerate}
\item Choose $T_i \in \Delta_\Omega.$
\item Define $\phi(T_i)$ as the set of triangles that share an edge with $T_i$. Note that $|\phi(T_i)|\leq 3, \ \ \forall T_i.$
\item Choose $T_j$ in $\phi(T_i)$. 
\item Step 4 as above.
\item  Repeat the previous 2 steps for all $T_j \in \sigma(T_i).$
\item Repeat the all the steps for all the triangles $T_i$ in the collection $\Delta_\Omega.$
\end{enumerate}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: 
%%% End:


==> sections/other_graph_extractions_2.tex <==
% !TEX program = pdflatex
% !TEX root = ../main.tex

%\section{The model}

\paragraph{A subgrid of the grid triangulation}
%The third  proposed way of constructing the graphs that we mentioned before is the following one.  


\begin{enumerate}
\item Choose $T_i \in \Delta_\Omega.$
\item Let $v,w,s$ be the grid nodes of $T_i$. If $\mu(T_i)\geq\delta $, then add $v,w,s$ to $V$ and $(v,w), (w,s),(s,v)$ to $E$.
\item Repeat the previous 2 steps for all the triangles $T_i$ in the collection $\Delta_\Omega.$
\end{enumerate}

These three rules result into three different network topologies as shown in Figure \ref{fig:Gextraction}.

\CDBcom{Cate stopped here}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: 
%%% End:


==> sections/ppd_model.tex <==
% !TEX program = pdflatex
% !TEX root = ../main.tex 

\paragraph{Dynamical formulation in discrete space}  \label{PPD}

Let $G=(V,E,w)$ be an undirected weighted graph. Denote as $s_0,s_{i}\in V$ the \textit{source} and \textit{sink} respectively, i.e. the nodes where the food is located. The edges $E$ of $G$ model the tubular channels of the mold. The weight $w:E\rightarrow \mathbb{R}$ is defined to be the \textit{length} function. For simplicity, we write $w(e)$ as $l_e, \ \forall e\in E$.  Let  $D,R,Q:E\times [0,\infty)\rightarrow \mathbb{R}$ be the \textit{diameter}, \textit{resistance} and \textit{protoplasmic flow} functions, resp.  For each edge $e$ and time $t$, we say that $D(e,t),\  R(e,t)$ and $Q(e,t)$ are the \textit{diameter}, the \textit{resistance} and the \textit{ protoplasmic flow through (or across)}  of the edge $e$ at time $t$, resp. From now on, we will use $D_e(t)$ to denote $D(e,t)$, $R_e(t)$ for $R(e,t)$ and $Q_e(t)$ for $Q(e,t)$.  Let $p:V\times [0,\infty)\rightarrow \mathbb{R}$ be the \textit{hydrostatic pressure} function. For any $v$ and $t$, there is a $p(v,t)$ (denoted as $p_v(t)$) that is the \textit{hydrostatic pressure} at node $v$ at time $t$. \CDBcom{TODO:shrink this paragraph}

The functions $D, Q, R$ and $p$ satisfy the following conditions:
\bea \label{PP}

\begin{array}{rll}
R_e(t)&= \dfrac{l_e}{D_e(t)}, \ \ \ \  &\forall e,\forall t, \\
Q_e(t)&=\dfrac{p_u(t)-p_v(t)}{R_e(t)},  \ &\forall e=(u,v), \forall t\\
\overset{\cdot}{D}_e(t)&= g\left(|Q_e(t)|\right)-D_e(t), \ \ &\forall e,\forall t, 
\end{array}
%\end{align}
\end{equation}
where $\overset{\cdot}{D}_e$ is $\frac{\partial}{\partial t}D(e,t)$. 

Defining $b:V\rightarrow \mathbb{R}$ as
$$
b(v)=\left\{
\begin{array}{rlc}
&1, &\text{ if } v=s_0,\\
-&1, &\text{ if } v=s_1, \\
&0, &\text{ otherwise,}
\end{array}
\right.
$$
and 
$$
\delta(v)=\{u\in V: \{v,u\}\in E \}, \ \ \forall v,
$$
to be the \textit{set of neighbours of} $v$. One last requirement for the model is to define a \textit{conservation law} for the flux $Q_{ij}$ as:
\begin{equation}\label{kirchhoff}
\underset{v\in \delta(u)}{\sum} Q_{\{u,v\}}(t)=b(u), \ \forall t
\end{equation}
for $u \in V.$

System \ref{PP} together with the conservation law \ref{kirchhoff} for all $u\in V$ are labeled as the \textit{Physarum Polycephalum Dynamics} (or \textit{PP Dynamics}). Note that once $D_e(t_0)$ ($t_0$, initial time: usually, $t_0=0$) is defined for all the edges $e$ and $p_v(t_0)$ is defined for $s_1$ (usually, $p_{s_1}(0)=0$), it is possible to solve the mentioned system in order to find the exact behaviour\footnote{According to the proposed model.}\footnote{More information about existence and uniqueness of solutions will be given later.} of the protoplasmic flow  inside the slime mold's body. The problem of finding $D_e$ (and thus $Q_e, \ R_e$ and $p_v$) for a set of initial time conditions on $D_e$ is known as the \textit{Physarum Polycephalum Dynamical problem} (or simply, \textit{PPD} problem). 


Note that system \ref{PP} could be generalized with the following modification
$$
\overset{\cdot}{D}_e(t)= g\left(|Q_e(t)|\right)-D_e(t), \ \ \forall e,t, 
$$
for $g:\mathbb{R}\rightarrow \mathbb{R}$. This leads to very different dynamics in terms of transport problems, but for the sake of simplicity, we will stick to the case $g(x)=x$. 

An informal equivalence of the PPD problem can be proposed in terms of electrical networks as follows.

Suppose that $D_e,\ Q_e, \ R_e$ and $p_v$ represent the \textit{conductance, current, resistance} and the \textit{potential}, resp. One can say that the system \ref{PP} represents the electrical dynamics in the network $G$, where a unitary current is forced from $s_0$ to $s_1$, and a flow conservation law is imposed at every vertex (\textit{Kirchhoff law} \ref{kirchhoff}). 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> sections/section_template.tex <==
% !TEX program = pdflatex
% !TEX root = main.tex



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> sections/steiner_problems.tex <==
% !TEX program = pdflatex
% !TEX root = main.tex files


\section{Steiner Problems}

Imagine we have four different points $v_1,v_2,v_3$ and $v_4$ in the plane, which are located in the vertices of the unit square, and we are interested in connecting them using a graph $G$ whose set of vertices $V$ is exactly our set of points $\{v_1, v_2, v_3,v_4\}$. In principle, we could propose a graph $G$ like the one in Figure \ref{st-graph} to solve the problem. 


\begin{figure}[h]
\centering
\includegraphics[scale=0.2]{figs/trees-for-steiner/1.png}
\caption{Graph with vertices $\{v_1,v_2,v_3,v_4\}$}\label{st-graph}
\end{figure}


Let's add now the following constraint: $G$ needs to have \textit{minimal total length}, i.e. 
$$
\sum_{e\in E(G)} l(e) \ 
$$
has to be as small as possible, where $l(e)$ denotes the length of the edge $e$.

Note that our graph $G$ does not satisfy this new constraint: its total length is equal to $2+\sqrt{2}$. Therefore, we need to propose a new graph $G'$ and check that it indeed has minimal total length. But, how can we do this? One way of approaching this new problem could be to look for all the possible graphs $G'$, computing the total length for each one of them, and then simply choosing the one with the required property. Figure \ref{trees} shows some of the trees $G'$ satisfying  $V(G)= \{v_1, v_2, v_3,v_4\}$. The reason why analyzing trees instead of all the graphs is enough to solve the problem will be given later on.
  
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/trees-for-steiner/1.png}
        \caption{$G_1$. T.L: $2+\sqrt{2}$}
        \label{fig:gull}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/trees-for-steiner/2.png}
        \caption{$G_2$. T.L: $2+\sqrt{2}$}
        \label{fig:tiger}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/trees-for-steiner/3.png}
        \caption{$G_3$. T.L: $2+\sqrt{2}$}
        \label{fig:mouse}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/trees-for-steiner/4.png}
        \caption{$G_4$. T.L: $2+\sqrt{2}$}
        \label{fig:gull}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/trees-for-steiner/5.png}
        \caption{$G_5$. T.L: $3$}
        \label{fig:tiger}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/trees-for-steiner/6.png}
        \caption{$G_6$. T.L: $3$}
        \label{fig:mouse}
    \end{subfigure}
    
    \caption{Trees connecting the vertices $\{v_1,v_2,v_3,v_4\}$ and their total length (T.L.)}\label{trees}
\end{figure}



As we can see, our set of candidates is very big (not only 6 but 16!\footnote{In general, the number of trees with $n$ vertices is $n^{n-2}$.}). Clearly, $G_5$ and $G_6$ have total minimum length among the ones showed, so it could be our solution. In fact, there are only 2 isomorphism\footnote{\href{https://en.wikipedia.org/wiki/Graph_isomorphism}{Graph isomorphisms.}} classes in the set of trees and these classes are invariant under total length, so instead of looking at all of the trees, it is enough to compare one representative of each one of the classes. As you might guess, both $G_5$ and $G_6$ are in the same isomorphism classes, and this is the one with the minimal total length.  

Consider now the following slight-modificated version of the previous problem: find a connected graph $G$ such that $V(G)\supset \{v_1,v_2,v_3,v_4\}$ and it has minimal total length. Now can do not have to connect the points by only using them as vertices but we can use some \textit{auxiliary points} to get shorter connections. A candidate for the solution of this problem is shown in Figure \ref{candidate}. The auxiliary vertex is located equidistant of the other vertices.


\begin{figure}[h]
\centering
\includegraphics[scale=0.23]{figs/trees-for-steiner/candidate.png}
\caption{Graph with auxiliary vertex $v_5$ and T.L., equal to $2\sqrt{2}$}\label{candidate}
\end{figure}

Using the same philosophy that we used before, we could try to solve these problems by looking for all the possible graphs $G$, computing their total length and finally, choosing the one with that minimizes this. Unfourtunately, this is not possible since now we are looking for nodes in an unconstrained space ($\mathbb{R}^2$) and the number of graphs we can build is infinite.  

This problem is known as the \textit{Euclidean Steiner Tree Problem} with \textit{four terminals}, and it was proposed by Jakob Steiner as a generalization of the Fermat-Torricelli problem, that consists in finding the point $y$ inside a triangle such that the total distance from $y$ to the three vertices of the triangle is the minimum possible. The most relevant first studies about this problem were published in 1811 by Joseph Diaz Gergonne\footnote{ \href{http://www.math.ucsd.edu/~ronspubs/14_02_Steiner.pdf}{On the History of the Euclidean Steiner Tree Problem}}.

We state the precise formulation of the problem mentioned before:

\textbf{Euclidean Steiner Tree (also known as \textit{Geometric Steiner Tree}) Problem:}

Given a set of $T\subset \mathbb{R}^2$ of $N$ points, find the graph $G=(V,E)$ such that $T\subset V$ and $G$ has minimal total length
$$
\sum_{e\in E} l(e) 
$$ 
where $l(e):=d_2(v,w)$ for $e=(v,w) \in E$. $l(e)$ is known as the \textit{length} of the edge $e$ and $d_2$ denotes the Euclidean distance. 



Euclidean Steiner Tree problems have been widely studied and many different approaches has been proposed to solve them. Due to the complexity of these problems (they are NP-complete), some authors have tried to look for suboptimal solutions, i.e. heuristics that give \textit{good} (in some sense) approximations to the solution.  

Imagine now that instead of using $\mathbb{R}^2$ as your domain, we move to a discrete space. This time we are interesting in connecting the nodes in our set $T$ using a graph $G$ as before, but this time the underlying structure on which we should build $G$ is a another graph $R$. In other words, the goal is to extract a subtree $G$ of $R$ containing $T$  with minimal total length.  This new problem is also a member of the family of Steiner problems, and it can be stated in the following terms:

\textbf{Graphical Steiner Tree (GSMT) Problem:} 

Given an undirected weighted graph $R=(V_R,E_R,w_R)$ and a set of nodes $T\subset V_R$, find the \textit{minimal} tree $G \subset R$\footnote{For graphs, $\subset$ denotes \textit{subgraph}.} that spans\footnote{A graph $G$ spans a set of vertices $W$ if $V(G)=W$.} $T$.  The graph $G$ is said to be \textit{minimal} if 
$$
G \in \underset{H\subset R}{\text{arg} \min} \ \sum_{e\in E(H)} w_R(e),
$$
i.e., $G$ minimizes the total weight. 

The set $T$ is known as the set of \textit{terminals}. The set $S(G):=V(G)- T$ is known as the set of \textit{steiner points} (they are the \textit{auxiliary points} that we mentioned before).

Even though both the graphical and the euclidean versions seem to be highly related, they have little in common in regards to the way they have been solved. Research on the GSMT problem has been done essentially through the following route: first, some exponential time exact algorthms for finding the optimal configuration were proposed. Afterwards, it was proved to be NP-complete\footnote{See Section (to be added) for a quick explanation about NP-problems.}. Lately, many heuristics and special cases have been developed. Nice references about the history of the Steiner Problems in general can be found in \href{https://onlinelibrary.wiley.com/doi/pdf/10.1002/net.3230220105}{Steiner Tree Problems} by F. K. Hwang and Dana S. Richards.

But what about the Graphical Steiner \textbf{Graph} Problem? Is it possible to reduce the complexity of the problem by removing the \textit{tree-like} condition? 
It was proved that if $w_R$ is a positive function then the optimal graph must be a tree ref ?.  We give now an intuitive explanation why this must be true: Imagine that $G$ is a solution of the GSMT, but $G$ is not a tree, then we can find a set of vertices $e_1,e_2,...,e_n$ in $G$ such that they form a cycle $C$ in $G$.  The total length of $G$ is the sum of the length of the edges in this cycle plus the ones that are not, i.e., 
$$
\sum_{1\leq i\leq n}w_R(e_i) + \sum_{e\notin C}w_R(e)
$$ 

but it is always possible to remove some edges in the cycle $C$ and get a new graph $G'$ that is stil connected and it also satisfies $V(G')=V(G)$ (Add ref). For the sake of simplicity, imagine that $C$ was the only cycle, therefore, $G'$ is a tree. The total length of $G'$ is now given by

$$
\sum_{e\in C'}w_R(e) + \sum_{e\notin C}w_R(e)
$$  
where $C'$ is $C$ without the removed edges, and clearly, this value is less than the total length of $G$, since 
$$
\sum_{1\leq i\leq n}w_R(e_i)  \geq \sum_{e\in C'}w_R(e).
$$

But this is contradictory, since we said before that $G$ was one solution of the GSMT problem and it was minimal in terms of total length. This contradiction comes from assuming that $G$ was not a tree. Thus, solutions of GSMT must be trees. This way is clear the even if we remove the tree condition on the GSMT problem, we will end up with solutions that are trees. 


We dedicate the remaining part of the section to explain the heuristic used to simplify our graphs. The algorithm\footnote{\href{https://dml.cz/bitstream/handle/10338.dmlcz/128936/MathSlov_31-1981-2_6.pdf}{A bound for the Steiner tree problem in graphs}.} was created by Jan Plesnik. Its implementation can be found in the Python package NetworkX. 

\subsubsection{Jan Plasnik's algorithm}\label{jan}


From now until the end of this section, let $R=(V_R,E_R,w_R)$ be an undirected weighted graph, with nonnegative edge weight function.  Let $T\subset V_R$ be the set of terminals. In this subsection we explain how to compute the \textit{metric closure graph} $\overline{R}$ of the graph $R$. This is a key part of Plasnik's algorithm.

Let $\overline{R}_T=(V,E,w_{\overline{R},T})$. The closure graph $\overline{R}$ is the complete graph\footnote{A \textbf{complete} graph is a graph in which every pair of distinct nodes is connected by a unique edge.} $K_{|T|}$, such that $V(\overline{R})=T$ and 
$$
w_{\overline{R},T}(e)=d(v,w), \ \ \forall (v,w)=e\in E(K_{|T|}),
$$

where $d$ is the shortest edge distance between $v$ and $w$ in $R$. 


In simple words, the metric closure graph $R$ of a graph is the complete graph built with the nodes of $R$ and whose weights are given by the shortest paths in the original graph. 


With this in mind, we can define Plasnik's algorithm. The steiner minimal tree generated by this algorithm will be denoted by $G$.  

\textbf{Algorithm:} Plasnik Minimal Steiner Tree.       

\textbf{Input:} A weighted undirected graph $R$ and a set of terminals $T$.  
    
\textbf{Output:} An approximation of a Steiner Tree $G$ of $R$.    
\begin{enumerate}
\item Construct the metric closure $\overline{R}_T$ of $R$
\item Find a weighted Minimum Spanning Tree\footnote{add this!} $H_T$ on $\overline{R}_T$
\item Initialize $V(G)=\varnothing$
\item \textbf{for} each edge $e=(v,w)\in E(G)$ in a depth-first-search order of $H_T$ \textbf{do}:
\begin{enumerate}
\item Find shortest path $P$ from $u$ to $v$ on $R$
\item \textbf{if} $P$ contains less than two vertices in $T$ \textbf{then}
\begin{itemize}
\item Add $P$ to $G$
\end{itemize}
\item \textbf{else}
\begin{itemize}
\item Let $p_1,p_2$ be the first and last resp. vertex in $P$. Add subpaths from $u$ to $p_1$ and from $p_2$ to $v$ to $G$. 
\end{itemize}
\end{enumerate}
\item Return $G$
\end{enumerate}


The time complexity of the algorithm is $O(|V(R)||T|^2)$, which comes essentially from the construction of the metric closure graph.  This algorithm generates an approximation $G$ of a Minimal Spanning Tree of $G$ whose total weight is within a $2-2/|T|$ factor of the weight of the actual Steiner Tree\ref{?}. To the best of our knowledge, the best approximation bound  is currently approximately equal to $1.39$\footnote{\href{http://people.idsia.ch/~grandoni/Pubblicazioni/BGRS12jacm.pdf}{Steiner Tree Approximation via Iterative Randomized Rounding}.} given by Byrka, Grandoni, Rothvo\ss, Sanit\`a \ref{?}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: 
%%% End:

